Diffusion on dynamic contact networks with indirect transmission links

Modelling diffusion processes on dynamic contact networks is an important research area for epidemiology, marketing, cybersecurity, and ecology. However, current diffusion models cannot capture transmissions occurring for indirect interactions. For example, an airborne infected individual releases infectious particles at locations that can suspend in the air and infect susceptible individuals arriving even after the infected individual left. Thus, current diffusion models miss transmissions during indirect interactions. In this thesis, a novel diffusion model called the same place different time transmission based diffusion (SPDT) is introduced to take into account the transmissions through indirect interactions. The behaviour of SPDT diffusion is analysed on real dynamic contact networks and a significant amplification in diffusion dynamics is observed. The SPDT model also introduces some novel behaviours different from current diffusion models. In this work, a new SPDT graph model is also developed to generate synthetic traces to explore SPDT diffusion in several scenarios. The analysis shows that the emergence of new diffusion becomes common thanks to the inclusion of indirect transmissions within the SPDT model. This work finally investigates how diffusion can be controlled and develops new methods to hinder diffusion.

==> Makefile <==
##################################################################
#
# LaTeX / PDFLaTeX Makefile
# (c) Tom Bobach 2007
# (c) Alexei Gilchrist 2008
#
# History:
#   24-09-2008  (AG) Stripped away some of the more dangerous code
#   17-07-2007  (TB) Added 2-levels of recursion for include checks
#   09-05-2007  (TB) Initial Version
#
# Disclaimer:
#   Use at your own risk.
#   I take no responsibility for this Makefile eating up your most
#   precious work, teaching your baby bad language or evoking evil
#   ghosts.
#
# What happens:
#   The current directory is searched for a *.tex file containing
#   the string "\documentclass"; this will be the main file.
#   All files included in the main file via "\include" will be
#   added to the source files.
#
#   If any of the input files contains the string "\bibliographystyle",
#   bibtex is invoked, the make dependency linked to the bib file found
#   in the "\bibliography{<file>}" entry.
#
# Usage:
#   make info        prints some info about the setup, what is considered
#                    the main file, what is the bibliography, what are
#                    the relevant images etc.
#   make clean       removes typical intermediate files.
#   make [pdf]       runs as stated in the beginning, assuming as target
#                    a pdf named after the main file.
#   make ps          like above, targeting a postscript
#   make dvi         like above, targeting a dvi
#   make view        opens kdvi with errors piped to /dev/null
#   make watch       checks every second for changes in *.tex, and *.bib
#
#
# TODO:
#   - support an arbitrary number of levels of recursion (currently 2)
#   - strip the comments from the texfile for every analysis of the text
#     (currently only done for bib file inclusion)
##################################################################

##################################################################
#   Main definitions - place your customizations here
##################################################################

MAINFILE=$(shell grep -l "\\\\documentclass" *.tex)

##################################################################
#   Some Definitions that should not need change
##################################################################

ifneq ($(words $(MAINFILE)),1)
$(error For automatic main file detection, only one .tex file can contain the "\documentclass" string. run make MAINFILE=<your mainfile>)
endif
# Currently, only two levels of recursion for included input is supported.
# If you need more, extend as you like after the scheme below.
TEXFILESPRE:=\
  $(shell grep "\\\\include{" $(MAINFILE) | sed 's/.*{\([^}]*\)}.*/\1/g') \
  $(shell egrep "\\\\input{.*}" $(MAINFILE) | sed 's/.*{\([^}]*\)}.*/\1/g')

ifneq ($(words $(TEXFILESPRE)),0)
  TEXFILES:=\
    $(MAINFILE:.tex=)\
    $(TEXFILESPRE)\
    $(shell grep "\\\\include{" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\)}.*/\1/g') \
    $(shell egrep "\\\\input{.*}" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\)}.*/\1/g')
else
  TEXFILES:=$(MAINFILE:.tex=) $(TEXFILESPRE)
endif


MUTE=@
SILENT=> /dev/null
VERYSILENT=1> /dev/null 2>/dev/null

MAKE=make --no-print-directory
LS=ls -1 --color=none
CP=cp

LATEX=pdflatex -shell-escape -interaction=nonstopmode
BIBTEX=bibtex

MSG_LAB_CHANGED="LaTeX Warning: Label(s) may have changed"
MSG_REF_UNDEFINED="LaTeX Warning: Reference.*undefined on input line.*"
MSG_CIT_UNDEFINED="LaTeX Warning: Citation.*undefined on input"

# strip all comments and extract the bibliography
FIND_BIB_FILE=$(shell \
	sed -e "s/\\\\%//g" $(1) | \
	sed -e "s/\([^%]*\).*/\1/g" | \
	grep "\\\\bibliography{"  | \
        sed 's/.*{\([^}^ ]*\)}.*/\1/g').bib

BIBFILE:=$(call FIND_BIB_FILE, $(TEXFILES:=.tex))
ifneq ($(BIBFILE),.bib)
  ifneq ($(wildcard *.bib),)
    BBL:=$(MAINFILE:.tex=.bbl)
  endif
endif


##################################################################
#   All the shell magic that helps us manage the twisted LaTeX
#   Compilation procedure
##################################################################


clear_valid=( [ ! -e .valid ] || $(RM) .valid )
check_undef_citations=\
  ( egrep $(MSG_CIT_UNDEFINED) $(MAINFILE:.tex=.log) > /dev/null )

# determine the changeset for citations
define check_citationchange
	(                                                \
	  [ -e .citations ] || touch .citations ;        \
	  ( grep "\\citation" $(MAINFILE:.tex=.aux)      \
		| sort                                   \
		| uniq                                   \
		| diff .citations -                      \
		> .citediff                              \
	  )                                              \
	)
endef

# exctract the citations from the aux file
define make_citations
	(                                                   \
	  (                                                 \
	    [ -e $(MAINFILE:.tex=.aux) ] &&                 \
	    ( echo "[info] Extracting citations...";        \
		grep "\\citation" $(MAINFILE:.tex=.aux)     \
		| sort                                      \
		| uniq                                      \
		> .citations                                \
	    )                                               \
	  )                                                 \
	  || touch .citations                               \
	)
endef

# comparing the citations in $(MAINFILE:.tex=.aux)
# against those in .citations.
# if there are differences, .citediff is changed.
define make_citediff
	(                                                     \
	  ( [ -e .citations ] || touch .citations ;           \
	    [ -e .citediff  ] || touch .citediff ;            \
	    echo "[info] Checking for changed Citations..." ; \
	    grep "\\citation" $(MAINFILE:.tex=.aux)           \
		| sort                                        \
		| uniq                                        \
		| diff .citations -                           \
	    > .citediff__                                     \
	  )                                                   \
	  || mv .citediff__ .citediff                         \
	)
endef

# compiles the document
# the file .valid is created if the compilation went without
# errors
define runtexonce
  ( 	                                                    \
    $(clear_valid);                                         \
    ( $(LATEX) $(MAINFILE) $(SILENT) &&                     \
      touch .valid );                                       \
    (                                                       \
      ( egrep $(MSG_REF_UNDEFINED) $(MAINFILE:.tex=.log)    \
        > .undefref ) ;                                     \
      ( egrep $(MSG_CIT_UNDEFINED) $(MAINFILE:.tex=.log)    \
        > .undefcit ) ;                                     \
      true                                                  \
    )                                                       \
  )
endef

# compile the document as many times as necessary to
# have cross-references right
define runtex
(                                                                      \
  echo "[info] Running tex...";                                        \
  $(runtexonce);                                                       \
  while( grep $(MSG_LAB_CHANGED) $(MAINFILE:.tex=.log) > /dev/null ) ; \
  do                                                                   \
      echo "[info] Rerunning tex...";                                  \
      $(runtexonce);                                                   \
  done                                                                 \
)
endef

##################################################################
#   Main compilation rules
##################################################################

pdf: $(MAINFILE:.tex=.pdf)

ps: $(MAINFILE:.tex=.dvi)

dvi: $(MAINFILE:.tex=.ps)



$(MAINFILE:.tex=.pdf): .compilesource
	$(MUTE)echo "[info] Created PDF."

# the dvi creation path invokes standard tex 
$(MAINFILE:.tex=.dvi): .force
	$(MUTE)$(MAKE) .compilesource \
		LATEX="latex -shell-escape -interaction=nonstopmode" 

%.ps: %.dvi
	$(MUTE)echo "[info] Converting DVI to PS"
	$(MUTE)dvips $< -o $@ $(VERYSILENT)

.compilesource: .force
	$(MUTE)$(MAKE) .valid
	$(MUTE)[ -z "$(BBL)" ] || $(MAKE) .citations
	$(MUTE)[ -e .valid ] || (                                    \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || echo "[Error] Could not make it work after 3 runs. Weird." ) \
	)
	$(MUTE) (                                                    \
           echo ; echo "Compilation Warnings:" ;                     \
	   grep "Warning" $(MAINFILE:.tex=.log) ;                    \
	   grep "Error" $(MAINFILE:.tex=.log) ;                      \
	   grep -A 1 "Undefined" $(MAINFILE:.tex=.log) || true       \
	)
	$(MUTE)[ ! -e $(MAINFILE:.tex=.bbl) ] || (                   \
	  echo ; echo "Bibtex Warnings:" ;                           \
	  grep "Warning" $(MAINFILE:.tex=.blg) ;                     \
	  grep "Error" $(MAINFILE:.tex=.blg) || true                 \
	)
	$(MUTE)[ -z "$(BBL)" -a -e .valid ] || [ -n "$(BBL)" -a -e .compiled ]


clean:
	$(MUTE)$(RM) *.bbl *.blg *.aux *.log *.toc *.lof *.lot
	$(MUTE)$(RM) .??*


view: $(MAINFILE:.tex=.pdf)
	kpdf $< > /dev/null 2>&1 &

viewdvi: $(MAINFILE:.tex=.dvi)
	kdvi $(<:.dvi=) > /dev/null 2>&1 &

viewps: $(MAINFILE:.tex=.ps)
	kghostview $< > /dev/null 2>&1 &

info:
	@echo Main file:    $(MAINFILE)
	@echo Input files:  $(TEXFILES:=.tex)
	@echo Bibliography: $(BIBFILE)

# just do one run...
.valid: $(TEXFILES:=.tex)
	$(MUTE)$(runtex)

# if citations changed since last run of bibtex, run it again.
.citations: .citediff $(BIBFILE)
	$(MUTE)[ ! -e .compiled ] || rm .compiled
	$(MUTE)(                         \
	  echo "[info] Running BibTex" ; \
	  bibtex $(MAINFILE:.tex=) $(SILENT)         \
	) && $(make_citations)
	$(MUTE) $(clear_valid)

.citediff: .force
	$(MUTE)$(make_citediff)

# run as long as necessary
.compiled: $(TEXFILES:=.tex) $(BBL) 
	$(MUTE)echo "Found undefined Citations, rerunning..."
	$(MUTE)$(runtex)
	$(MUTE)$(check_undef_citations) || touch .compiled

.force:

define runwatch
  $(MUTE)CHANGE=true && while true ; \
  do       \
    if $$CHANGE ; then                             \
      echo;                             \
      echo "#######################################"; \
      echo "#    RUNNING MAKE                     #"; \
      echo "#######################################"; \
      echo;                                       \
      make;                                        \
      for i in $(TEXFILES:=*.tex) $(BIBFILE) ; do   \
        touch .$$i -r $$i;                         \
      done;                                        \
      CHANGE=false;                                \
    fi;                                            \
    sleep 2;                                       \
    echo 'tic' ; \
    for i in $(TEXFILES:=*.tex) $(BIBFILE) ; do     \
      if [ .$$i -ot $$i ] ; then                   \
        CHANGE=true;                               \
      fi                                           \
    done ;                                         \
  done
endef

watch:
	$(runwatch)


==> conold.tex <==
%------------------------------------------------------
% QUOTE
% If you really feel like adding a quote
% to your page, uncomment out the following.
%------------------------------------------------------
%\begin{savequote}[45mm]
%When theory and experiment agree, 
%that is the time to be especially suspicious. 
%\qauthor{Niels Bohr}
%\end{savequote}
%------------------------------------------------------
% QUOTE
% If you really feel like adding a quote
% to your page, uncomment out the previous.
%------------------------------------------------------


\chapter{Conclusion}
The main goal of this thesis is to investigate how the inclusion of indirect transmission opportunities influence diffusion phenomena on dynamic contact networks. In particular, this thesis has developed a diffusion model called the same place different time transmission based diffusion model (SPDT diffusion) and a graph model called SPDT graph for investigating diffusion phenomena with indirect transmission links. Then, SPDT diffusion behaviours and it's controlling on dynamic contact networks are explored. This chapter describes the main findings, limitations of conducted research and future research directions on SPDT diffusion. The discussion is derived by the research questions which are discussed in the introduction chapter. 

\subsubsection{SPDT diffusion model}
Current diffusion model cannot properly capture indirect transmission opportunities of contagious items in the diffusion dynamics. A novel diffusion model called the same palace different time transmission based diffusion (SPDT diffusion) has been developed in Chapter 3 to fill this gap. Therefore, the SPDT model can produce diffusion dynamics that include both the direct links, where both infected and susceptible individuals are present at a location, and indirect links, where susceptible individuals visit the locations where an infected individual has been. The transmission links in SPDT model are called SPDT links and are created through space and time. A key feature of the SPDT link is that the transmission probability of contagious items decay over time if it has indirect transmission link. A new infection risk assessment method is developed for SPDT diffusion model to asses the transmission probability through SPDT links. Thus, the SPDT diffusion model accounts for the arrival and departure time of both susceptible and infected individuals at the interaction locations and calculates the transmission probability of contagious items accordingly. The risk assessment method defines a particle decay rate which reflects the impacts of all kinds of removal of contagious items from the interaction location against a particle generation rate. In the SPDT model, therefore, heterogeneous transmission probabilities for SPDT links can be assigned by a random value of particle decay rate and having different arrival and departure times of both susceptible and infected individuals. 

The inclusion of indirect transmission with the SPDT diffusion model introduces a new dimension in network dynamics where the underlying contact dynamic varies with particle decay rates. This is because the length of time contagious items persist in the media varies with particle decay rates. Therefore, the number of susceptible individuals that will be connected with an infected individual for a visit to a location often depends on this length of time. As a result, the connectivity in the network modifies according to decay rates $r_t$ and hence the speed of contagious items spreading changes. For example, the network connectivity becomes denser at lower $r_t$ and contagious items spread faster. Investigations in Chapter 3 shows that there is a threshold value of $r_t$ above which the disease prevalence increases in the networks. Otherwise, the disease dies out shortly. Impact of decay rate is stronger in the dense networks compared to that of sparse networks. This is because the effect of $r_t$ is amplified with the more links density of dense networks. Disease parameters such as infectiousness of disease and recovery rate from the disease also vary the influence of decay rate $r_t$. The analysis shows that the impact of SPDT links is not reproducible with the direct SPST links as the decay properties of indirect links are not captured with direct links.

The SPDT diffusion model captures realistic disease reproduction due to including indirect transmission links. In addition, changes in SPDT diffusion dynamics according to decay rates $r_t$ can be applied to model the seasonal variations in infectious disease spreading. For example, incidence of influenza A increases in winter when infectious particles has more opportunities to suspend in the air due to low humidity. Therefore, infectious particles stay longer in the air and cause more infections. The SPDT model also can be used to study the spreading of information in online social networks (OSN). For example, the attraction to a message posted on the Facebook wall of a user decays with time. Therefore, this link for transmitting message has decay properties that are similar to indirect links in the SPDT model. The model can also be applied for queen message distribution in ant colonies. 

There are some limitations for analysing SPDT diffusion. The decay rates combine all removal processes of contagious items. However, the removal processes of contagious items or decay rates of SPDT links are complex as it is determined by several other factors such as weather conditions, properties of contagious items and properties of transmission media where it is spreading. It is often required to combine the impacts of all these processes separately. In the simulations, it is assumed that individuals are homogeneously susceptible. However, it is not true in reality and individual heterogeneity may change the diffusion dynamics. In addition, the contact information is aggregated over one day and it is assumed that this will produce the similar results of the separate contact information. For simulating disease spreading, the empirical contact networks constructed by the Momo users are used. This provides the partial contact information of a real world scenarios. Applying complete information may bring new diffusion dynamics. In constructing contact networks, if neighbour individuals visit the location within 3 hours of departure of infected individuals, the SPDT links are created. However, there are some diffusion process such as vector-borne disease that can transit disease for a few days. The diffusion behaviours obtained in this case may vary as a result. In spite of all these limitations, the SPDT diffusion model developed reveals some new diffusion behaviours for a class of diffusion phenomena that is not widely discussed in the literature.

%\textbf{Future research directions}\\
The SPDT diffusion model introduces interesting and potential research problems in the field of diffusion study. Exploration of individual-level movement data allows the researcher to develop data-driven diffusion model. However, the obtained results are often validated with the analytical model. Thus, it is important to develop a mathematical model for SPDT diffusion. In this study, the realistic disease parameters from the literature are used to simulate the disease spreading. It would be an interesting research direction to collect real disease incidence and comparing the simulation results with them. This thesis mainly focuses on exploring diffusion behaviours with the inclusion of indirect transmission links. This model can be studied in other scenarios such as message dissemination in OSN.

\subsubsection{SPDT graph model}
The current exploration of technology offers a gathering of mass data on individual behaviours which allows modelling of diffusion processes on empirical contact data. However, these data still hold limitations such as it is not easily available due to privacy, often misses some part of real-world data etc. Therefore, the data-driven method based on the empirical data sets may mislead the conclusion of a diffusion process. In addition, it is often hard to study if-else scenarios elaborately with the empirical data sets. Therefore, the alternative approach is often to use synthetic contact data generated by graph models to study and validate the results of empirical sets. The current graph models can generate contact networks where the links are created for direct interactions only. Thus, a graph model called SPDT graph is developed to create links for both direct and indirect interactions. 


The SPDT graph is developed based on the principle of activity driven time-varying network modelling. The idea of activating a node at a time step with a probability is extended to activate node for a consecutive time step (active period) to mimic the stay of individuals at a location. The other extension is to create a node copy for each activation and allow them to create direct and indirect links with other nodes. Then, an SPDT graph generation method is developed. This method allows one to fit the model parameters with real data. The graph model fitting methods are developed using maximum likelihood estimators. The model are validated comparing the network properties with that of real data and studying the simulation capability of SPDT process. 

The graph model can generate various SPDT contact networks varying the model parameters that can be used to explore SPDT diffusion processes. The graph model can also generate SPST contact networks for co-location direct interactions. The generated networks can be applied to study message dissemination in social networks, developing co-operation based applications, and same interest based applications as the active periods capturing group meeting of individuals. The other interesting application of SPDT graph can be to model diffusion on multiple social network platforms. A user can be active in multiple social networks and interact with friends which can be captured by the concept of active copy which play roles separately in the model. 

There are several interesting directions for future development of the developed graph model. For simplicity, it is assumed that the maximum link creation delay is constant. Thus, the model might miss some of the contacts that are created after that period and their impact on diffusion. The network generation process can be improved to include the unlimited link creation delay which is now limited to 3 hours. The model currently aggregates the node states of the basic activity driven network model. It will be important in the future to quantify the effect of this aggregation simplification along with other simple assumptions that may affect the model's resolution and representativeness. The critical conditions for network stability should also be studied further. This will increase the applicability of networks for a wide range of SPDT diffusion study.

\subsubsection{Indirect link potential}
It is seen in Chapter 3 that the inclusion of indirect links amplifies the diffusion dynamics. Then, the potentialities of the indirect links are analysed in Chapter 5. The interaction patterns define the network properties. The previous studies have focused on the networks properties and their impact on diffusion based on the direct transmission links. However, the network properties in the SPDT diffusion model is built based on the indirect transmission links along with the direct transmission links. Therefore, they have different impacts on diffusion dynamics. A node is connected with their neighbouring nodes through links which form the local contact structure and its position in the networks. The spreading of contagious items from a node depends on the local contact structure and its position in the network. Thus, it is studied in this chapter how the indirect links are potential to form local structure and changing the position of nodes in a network. Hence, the spreading potential of nodes changes and the emergence of contagious items alter. 


The SPDT model introduces a new property in the network through hidden spreader nodes, who does not have direct transmission links during their infectious periods. The spreading potential of nodes in SPDT network is studied through these hidden spreaders as they do not transmit disease through direct links. This can indicate the transmission potentiality of the indirect transmission links. The analysis shows that the indirect links have the same potential to that of direct transmission links. The interesting finding is that hidden spreader node can be supper-spreader which are assumed to have zero spreading potential. This chapter also reveal that the networks with only hidden spreaders can do outbreak of significant sizes. This indicates that if face-to-face meeting is restricted during outbreaks, there might be disease spreading through co-location indirect interactions. The other finding of this chapter is that the number of super-spreaders increases significantly in SPDT model due to including indirect transmission links. Therefore, the likelihood of emerging infectious disease becomes eases. This also makes harder to control the spreading of diseases.

The impacts of indirect links are studied through spreading potential. It is not studied the enhancement in a specific network property and the correlation between them and resultant diffusion. The spreading potential is studied through hidden spreaders. However, it was unknown how the neighbour nodes are connected with their neighbours and their impacts on diffusion. If the neighbours are connected with the neighbours through direct links, the spreading potential of the studied node might have overestimated. However, the study of the network with hidden spreaders shows that the hidden spreaders can be super-spreaders with significant outbreak sizes which is almost half of the non-hidden super-spreader. This also indicates the same potentiality for both direct and indirect links. The nodes are classified into five groups to study the boasting in super-spreader behaviours. The varies in class range may vary the results.

There are several interesting research issues on networks properties with indirect links. The creation of indirect links in SPDT model for visiting the same locations provide opportunities to connect one individual to many other individuals comparing to that in the SPST model. Thus, the community structure is changed in the SPDT model. It is widely discussed in the literature that the community structure has a strong influence on diffusion dynamics. It would be interesting to know how the community structure is changed in the SPDT model and impacts diffusion dynamics. The indirect links creation opportunities also change in the temporal paths in SPDT model than that of SPST model. Thus, the other interesting direction of research is to study in the temporal properties and their impacts on diffusion dynamic in SPDT model.  


\subsubsection{Controlling SPDT diffusion}
Controlling SPDT diffusion is one of the key application of diffusion study. In Chapter 6, controlling of SPDT diffusion is studied through vaccination strategies. The study of Chapter 5 shows that the indirect links have profound impacts on shaping the SPDT diffusion phenomena on dynamic contact networks. The control strategies based on the direct transmission links fails to control diffusion on the SPDT contact networks. The other challenges in controlling SPDT diffusion is that the indirect interactions are not visible to the interacted individuals. Thus, an individual movement based vaccination (IMV) strategies are in Chapter 6 where individuals (nodes) are ranked based on their movement behaviours. This strategy depends on local contact information and does not require global information. The other important features of IMV strategy is that it uses approximate information instead of exact contact information. Thus, the individuals are not required to provide accurate information which is impossible in reality.

The proposed IMV strategy is analysed in both preventive and post-outbreak vaccination scenarios and performance is compared with three other popular vaccination strategies. In the preventive vaccination scenarios, the proposed IMV strategy shows better performance than the other local information based strategies such as random vaccination (RV) and acquaintance vaccination (AV). With the coarse-grained information, IMV strategies achieve the efficiency of degree based vaccination strategies. The analysis shows that RV strategy requires to 70\% of nodes to be vaccinated and AV strategy requires 40\% of nodes to be vaccinated for safe prevention whereas IMV strategy requires only 2\% nodes to be vaccinated. The vaccination strategies are also studied against the scenarios where contact information is only available for a proportion of nodes. For 50\% of nodes information, the RV and AV strategy could not prevent disease spreading with vaccinating all nodes given their contact information. However, IMV strategy can prevent disease spreading with vaccinating 35\% of nodes. 

Similar to preventive vaccination, IMV strategy also shows a better performance in post-outbreak scenarios. In the population level vaccination, IMV strategy contains disease within the outbreak of 1K infections with vaccinating 6\% of nodes while RV strategy requires vaccination of 55\% nodes and AV requires 35\%. For the scenarios with limited information availability, the spreading of disease is contained with more efficiency by IMV strategies. No vaccination strategy can contain disease outbreak properly with the information availability of 25\% nodes. The AV and RV strategy requires information of at least 75\% of nodes. However, IMV strategy can work for the information of 50\% nodes. The requirements of vaccinating 6\% nodes in IMV reduces to 0.5\% nodes if the vaccination is applied through node level vaccination (ring vaccinating). The node level vaccination performs well with the limitation of identifying infected nodes as well. For identifying proportion $F=0.25$ to $F=1$, the performance of IMV and DV strategy does not change while RV strategy is strongly affected.  



Implementation of vaccination also defines the performance of the strategies. For example, strategy provides better performance if vaccination implemented community or regional wise. Instead of vaccinating many individuals from the same community, it may be more efficient vaccinate individuals from different community or region. This can a potential research direction for study SPDT diffusion control. The proposed strategy is not studied comparing to strategies integrating temporal information. Performance of control strategy can be studied with temporal information based methods. For the post-outbreak scenarios, closures methods (school close, popular location closes) are widely studied for post-outbreak vaccinations. Thus, the performance of IMV strategy can be compared with these closure methods.


\subsubsection{Thesis summary}
This thesis study a class of diffusion processes where contagious items have opportunities to spread through indirect transmission links along with direct transmission links. A new diffusion model called the same place different time transmission based diffusion (SPDT diffusion) is developed to capture indirect transmission in diffusion dynamics on dynamic contact networks. Data-driven approaches are applied to explore the SPDT diffusion dynamic behaviours using the empirical contact data provided by the users of a social networking application Momo. The SPDT diffusion dynamics analysis shows different behaviours to that of traditional same place same time transmission based diffusion (SPST diffusion). Indirect transmission links characterise the new diffusion behaviours of SPDT model comparing to SPST model. It is also found that SPDT diffusion dynamics are not reproducible with the SPST model. Then, this thesis focuses to develop a graph model called SPDT graph which can generate contact networks with direct and indirect transmission links among nodes. SPDT graph model is developed based on the principle of activity driven time-varying network modelling and fitted with real network contact properties. Generated contact networks by the developed graph model can simulate the SPDT diffusion and reproduce diffusion dynamics of real contact networks. Using the generated synthetic networks and real contact networks, the potentiality of indirect links and the behaviours of hidden spreaders, the node having only indirect links during their infectious period, are analysed in details. This shows that the indirect links assume the similar potential of direct transmission links and disease can emerge from hidden spreaders that are assumed to have zero spreading potential in the current SPST model. Finally, controlling of SPDT diffusion is studied using vaccination strategies. A new vaccination strategy is proposed based on the individual movement behaviours for controlling SPDT diffusion on dynamic contact networks. The proposed vaccination strategy substantially improves the efficiency of local information based vaccination strategy and achieves the efficiency of global information-based strategy. It is found that the proposed strategy perform well under the constraint of information availability.




